Generative AI in Embodied Systems: System-Level Analysis of Performance, Efficiency and Scalability

Embodied systems, where generative autonomous agents engage with the physical world through integrated perception, cognition, action, and advanced reasoning powered by large language models (LLMs), hold immense potential for addressing complex, long-horizon, multi-objective tasks in real-world environments. However, deploying these systems remains challenging due to prolonged runtime latency, limited scalability, and heightened sensitivity, leading to significant system inefficiencies. In this paper, we aim to understand the workload characteristics of embodied agent systems and explore optimization solutions. We systematically categorize these systems into four paradigms and conduct benchmarking studies to evaluate their task performance and system efficiency across various modules, agent scales, and embodied tasks. Our benchmarking studies uncover critical challenges, such as prolonged planning and communication latency, redundant agent interactions, complex low-level control mechanisms, memory inconsistencies, exploding prompt lengths, sensitivity to self-correction and execution, sharp declines in success rates, and reduced collaboration efficiency as agent numbers increase. Leveraging these profiling insights, we suggest system optimization strategies to improve the performance, efficiency, and scalability of embodied agents across different paradigms. This paper presents the first system-level analysis of embodied AI agents, and explores opportunities for advancing future embodied system design.

==> Sections/1_Introduction.tex <==
\section{Introduction}
\label{sec:intro}

% what is embodied AI agent system?
Embodied AI systems represent intelligent agents that interact with the physical world through perception, cognition, and action to accomplish complex tasks~\cite{duan2022survey,xu2024survey,liu2024aligning}. These systems integrate advanced cognitive frameworks with environmental sensing and task execution to navigate long-horizon multi-objective challenges, such as motion planning and autonomous decision-making. Recently, large language models (LLMs) have been increasingly incorporated into embodied AI systems to enhance planning, communication, and reasoning capabilities in dynamic and uncertain environments.

% advantages
Embodied AI agents hold significant potential for real-world applications, including robotics, autonomous vehicles, and collaborative multi-agent systems. By combining high-level reasoning from LLMs with precise low-level execution, these systems enable robust and adaptive behaviors in complex tasks that require continuous engagement with the environment. 
They have demonstrated superior capabilities in long-horizon multi-objective tasks across various domains. For example, CoELA~\cite{zhang2024building} improves success rate by 23\% in complex object transportation, table setting, and dish-washing human-agent interaction tasks across benchmarks.

% challenges
Despite their promising application potentials, embodied AI systems face critical challenges. First, the \emph{high computational latency} in long-horizon tasks arises from repeated inference runs and complex planning processes. Second, \emph{system inefficiencies}, such as redundant communication and sequential processing, lead to increased runtime and reduced task efficiency. Third, the \emph{scalability of multi-agent systems} is hindered by communication bottlenecks, memory overhead, and the exponential growth of action interdependencies as the number of agents increases. Finally, \emph{local model limitations and memory inconsistencies} further degrade system performance in large-scale tasks. For instance, we observe that current embodied AI agent systems, such as CoELA~\cite{zhang2024building}, COMBO~\cite{zhang2024combo}, and MindAgent~\cite{gong2023mindagent}, are highly inefficient, requiring 18, 23, and 21 minutes, respectively, even on desktop GPUs, to complete a single long-horizon multi-objective task.

In this work, we aim to comprehensively analyze the latency, efficiency, and scalability of embodied AI systems from the \emph{computing and system perspective}. We set out to answer three key research questions: \emph{What are the fundamental building blocks and paradigms of embodied systems? What are the system characteristics and sources of inefficiencies in embodied agents? How can the efficiency and scalability of embodied systems be improved?}
% Our study focuses on identifying key performance bottlenecks and profiling various components and explore optimization opportunities to enhance system efficiency and scalability.

We first present a systematic categorization of embodied AI systems (Sec.~\ref{sec:paradigm}). We illustrate the fundamental building blocks - sensing, planning, memory, communication, reflection, and execution - that constitute embodied agents, and categorize them into single-agent and multi-agent systems. Single-agent systems adopt either a modularized paradigm which integrates building blocks, or an end-to-end paradigm where pre-trained models directly output agent actions. Multi-agent systems can be categorized into centralized and decentralized paradigms, based on how agents cooperate and communicate.
% where a central agent coordinates all agents' plans, and decentralized paradigms, where agents operate independently and communicate to collaborate.

To uncover system inefficiencies, we then conduct a comprehensive profiling of 14 representative embodied AI systems (Secs.~\ref{sec:selected_system}, \ref{sec:profiling}, \ref{sec:profiling_scalability}, \ref{sec:profiling_sensitivity}). Our workload characterization provides new observations and insights, including the following:

\begin{itemize}
    \item Embodied AI agent systems typically exhibit long runtime latency on long-horizon multi-objective tasks, prohibiting them from real-time applications.
    \item LLM-based planning and communication dominate the latency while low-level execution also contributes notable delays. Sequential processing and redundant communication result in cumulative latency and reduced cooperation efficiency.
    \item Larger memory modules improve embodied task performance but introduce retrieval latency and inconsistencies.
    \item Token length increases over time due to redundant retrieval and concatenated multi-agent dialogues, raising costs and reducing LLM reasoning capability.
    \item Multi-agent embodied systems face performance drops in centralized paradigms and latency bottlenecks in decentralized paradigms.
    \item Reflection improves error correction with minimal overhead, while execution modules are indispensable for task completion and precision.
    
\end{itemize}

Inspired by our workload profiling insights, we recommend several cross-layer software and hardware optimization solutions to improve the efficiency and scalability of embodied AI systems (Secs.~\ref{sec:profiling}, \ref{sec:profiling_scalability}, \ref{sec:profiling_sensitivity}). Finally, we explore the research opportunities in embodied AI agent computing and share our outlook on the road ahead (Sec.~\ref{sec:opportunity}).

To the best of our knowledge, this is one of the \emph{first} works to assess the efficiency of embodied AI systems from computing and system perspectives. We aim to inspire the design of next-generation embodied AI systems through synergistic advancements in models, software, and computing architectures.

% benchmark,
% analytical system,
% proxy load generator,


==> Sections/5_System_Implication.tex <==
\section{System Implication}
\label{sec:implication}


==> Sections/6_Opportunity.tex <==
\section{Outlook and Research Opportunities}
\label{sec:opportunity}

In this section, we explore the challenges and opportunities for advancing embodied AI robotic systems, outlining our vision for the future from a computing systems perspective.

\textbf{Layered software stack for embodied AI flexibility.} Embodied AI systems need to integrate a wide range of functionalities, from environmental perception and physical interaction to executing complex tasks. This complexity is further amplified by the need for a versatile architecture that can support various agent forms and tasks, making seamless integration across different components difficult. However, this presents a unique opportunity to develop a layered software architecture to manage complexity and improve system flexibility~\cite{liu2024building}. The layered structure would include a \emph{control adaptation layer} to simplify hardware integration, a \emph{core robotic functions layer} to handle essential operations, and an \emph{application layer} to enable sophisticated AI application development. This architecture can create a more adaptable and efficient software ecosystem for embodied AI.

\textbf{Integrated computing architecture for embodied AI efficiency.} Current computing infrastructures fall short in addressing the rigorous demands of real-time data processing, energy efficiency, and reliability that embodied robots need to function optimally in dynamic environments. This gap highlights the necessity for novel architectures that enhance computational efficiency in embodied AI systems. \emph{An effective architecture should seamlessly integrate multimodal sensors, deliver robust computational support for core robotic tasks, and facilitate real-time processing of large, model-driven applications}~\cite{liu2024building,hao2024orianna,krishnan2022automatic}. By designing systems that synchronize multimodal sensor data accurately, improve computational performance through dataflow optimization, and enable real-time execution of large visual language models on edge devices, researchers can greatly enhance the efficiency and responsiveness of embodied AI in practical applications.

\textbf{Data-centric design automation for embodied AI scalability.} The progress and optimization of embodied AI systems are highly dependent on the availability and use of \emph{extensive, high-quality datasets}, which are often difficult to gather. The diverse and complex nature of real-world settings, along with the logistical and technical barriers in data collection, limits the ability of embodied robots to efficiently learn and adapt. One promising solution is \emph{design automation}, which combines both synthetic and real-world data~\cite{yu2023autonomous}. By training models in simulated environments with synthetic data, and subsequently fine-tuning them using smaller amounts of real-world information, researchers can facilitate the development of scalable embodied AI systems. Building a design automation pipeline, particularly using digital twin simulations, offers an effective way to overcome the data limitations and improve the adaptability and scalability of embodied AI. \yd{Maybe also mention modularity / compositionality as another way to potentially reduce the amount of data, since you only need data from the modules?}

% \textbf{Standards framework for embodied AI safety and reliability.}
% This complexity of embodied AI system underscores the imperative need for standards framework to ensure safety and reliability, especially given their close interaction with humans in complex environments. \emph{Safety} is paramount in embodied AI systems because any malfunction or unintended behavior can result in serious injury or harm to humans. Ensuring safety involves preventing accidents through reliable hardware and software integration, implementing fail-safes and emergency stop mechanisms, and adhering to stringent safety standards.
% \emph{Reliability}, equally crucial to embodied AI systems, depends on durable components and consistent performance across different conditions, with stable software that operates without errors or crashes. Fault tolerance is also vital, allowing the system to recover from errors with minimal disruption to performance and safety.
% Inspired from safety and reliability standards framework in autonomous vehicle (e.g., ISO 26262, ISO 21434), it is imperative to establish comprehensive standards frameworks for embodied AI systems~\cite{liu2024building2}. The standard would enhance safety and reliability, facilitating the widespread adoption and effective deployment of embodied AI technologies in diverse scenarios, ultimately building trust and advancing the field.

==> Tables/profiling_metric.tex <==
\begin{table}[t!]
\centering
\caption{\textbf{Benchmark Metrics.} Task performance and system efficiency metrics for embodied workload characterization study.}
\resizebox{.8\columnwidth}{!}{%
    \begin{tabular}{ll}
        \toprule
        \textbf{Metric} & \textbf{Description} \\ 
        \midrule
        \textbf{Task Performance} & Measured by the \emph{success rate} metric. \\ 
        \textbf{Runtime Latency} & Latency per step for a task. \\ 
        \textbf{Average Steps} & Average number of steps taken per task. \\ 
        \bottomrule
\end{tabular}
}
\vspace{-10pt}
\label{tab:profiling_metrics}
\end{table}


% \begin{table}[h!]
%     \centering
%     \caption{Profiling Metrics for Task Performance and System Efficiency}
%     \label{tab:profiling_metrics}
%     \begin{tabular}{ll}
%         \toprule
%         \textbf{Metric} & \textbf{Description} \\ 
%         \midrule
%         \textbf{Task Performance} & Measured by the \emph{success rate} metric. \\ 
%         \textbf{Runtime Latency} & Latency per step for a task. \\ 
%         \textbf{Average Steps} & Average number of steps taken per task. \\ 
%         \bottomrule
%     \end{tabular}
% \end{table}

==> Tables/workload_paradigm.tex <==
\begin{table}[t!]
\centering
\caption{\textbf{Embodied AI Agent Systems.} Categorization of recent embodied AI agent systems into four paradigms with their computing module compositions. Action types V, T, E represent virtual action, tool usage, and physical action, respectively. \yd{For end to end paradigms, all the papers are from the same group of people. Could consider removing some of the papers and add other papers like 3D-VLA or Diffusion Policy or some autonomous driving vla models (i.e. maybe GAIA?) from other people.}}
\renewcommand*{\arraystretch}{1.15} % Adjust row height
\setlength\tabcolsep{1pt} % Adjust column separation
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|c|c|cccccc|c}
% \toprule
\hline
\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{System Paradigm}}} & \multirow{2}{*}{\textbf{Workloads}} & \multicolumn{6}{c|}{\textbf{Computing Modules}} & \multirow{2}{*} {\textbf{Embodied Type}} \\
\cline{4-9}
\multicolumn{2}{c|}{} & & Sense & Plan & Comm. & Mem. & Refl. & Exec.  \\ \hline
% \midrule

% ================= Single Agent, Modularized ==================
\multirow{25}{*}{\begin{tabular}{c}Single-\\Agent\end{tabular}} 
& \multirow{20}{*}{\begin{tabular}{c}Modularized\\Paradigm\end{tabular}} 
& Mobile-Agent \cite{wang2024mobile} & \green{\cmark} & \green{\cmark} & \color{orange}{\xmark} & \color{orange}{\xmark} & \green{\cmark} & \green{\cmark} & Device Control (T) \\ \cline{3-10}
& & AppAgent \cite{zhang2023appagent} & \green{\cmark} & \green{\cmark} & \color{orange}{\xmark} & \color{orange}{\xmark} & \color{orange}{\xmark} & \green{\cmark} & Device Control (T) \\ \cline{3-10}
& & PDDL \cite{guan2023leveraging} & \color{orange}{\xmark} & \green{\cmark} & \color{orange}{\xmark} & \color{orange}{\xmark} & \green{\cmark} & \color{orange}{\xmark} & Simulation (V) \\ \cline{3-10}
& & RoboGPT \cite{chen2023robogpt} & \green{\cmark} & \green{\cmark} & \color{orange}{\xmark} & \color{orange}{\xmark} & \color{orange}{\xmark} & \green{\cmark} & Simulation (V) \\ \cline{3-10}
& & VOYAGER \cite{wang2023voyager} & \color{orange}{\xmark} & \green{\cmark} & \color{orange}{\xmark} & \green{\cmark} & \green{\cmark} & \green{\cmark} & Simulation (V) \\ \cline{3-10}
& & MP5 \cite{qin2024mp5}& \green{\cmark} & \green{\cmark} & \color{orange}{\xmark} & \color{orange}{\xmark} & \green{\cmark} & \green{\cmark}  & Simulation (V) \\ \cline{3-10}
& & RILA \cite{yang2024rila} & \green{\cmark} & \green{\cmark} & \color{orange}{\xmark} & \green{\cmark} & \green{\cmark} & \green{\cmark} & Navigation (V) \\ \cline{3-10}
& & CRADLE \cite{tan2024towards} & \green{\cmark} & \green{\cmark} & \color{orange}{\xmark} & \green{\cmark} & \green{\cmark} & \green{\cmark} & Device Control (T) \\ \cline{3-10}
& & STEVE \cite{zhao2025see} & \green{\cmark} & \green{\cmark} & \color{orange}{\xmark} & \color{orange}{\xmark} & \color{orange}{\xmark} & \green{\cmark} & Simulation (V) \\ \cline{3-10}
& & DEPS \cite{wang2023describe} & \green{\cmark} & \green{\cmark} & \color{orange}{\xmark} & \color{orange}{\xmark} & \green{\cmark} & \green{\cmark} & Simulation (V) \\ \cline{3-10}
& & JARVIS-1 \cite{wang2024jarvis} & \green{\cmark} & \green{\cmark} & \color{orange}{\xmark} & \green{\cmark} & \green{\cmark} & \green{\cmark} & Simulation (V) \\ \cline{3-10}
& & FILM \cite{min2021film} & \green{\cmark} & \green{\cmark} & \color{orange}{\xmark} & \color{orange}{\xmark} & \color{orange}{\xmark} & \green{\cmark} & Simulation (V) \\ \cline{3-10}
& & LLM-Planner \cite{song2023llm} & \color{orange}{\xmark} & \green{\cmark} & \color{orange}{\xmark} & \color{orange}{\xmark} & \green{\cmark} & \green{\cmark} & Simulation (V) \\ \cline{3-10}
& & EmbodiedGPT \cite{mu2024embodiedgpt} & \green{\cmark} & \green{\cmark} & \color{orange}{\xmark} & \color{orange}{\xmark} & \color{orange}{\xmark} & \green{\cmark}  & Simulation (V) \\ \cline{3-10}
& & Dadu-E \cite{sun2024dadu} & \green{\cmark} & \green{\cmark} & \color{orange}{\xmark} & \green{\cmark} & \green{\cmark} & \green{\cmark} & Simulation (V) \\ \cline{3-10}
& & MINEDOJO \cite{fan2022minedojo} & \green{\cmark} & \green{\cmark} & \color{orange}{\xmark} & \green{\cmark} & \color{orange}{\xmark} & \green{\cmark}  & Simulation (V) \\ \cline{3-10}
& & Luban \cite{guo2024luban} & \green{\cmark} & \green{\cmark} & \color{orange}{\xmark} & \green{\cmark} & \green{\cmark} & \green{\cmark} & Simulation (V) \\ \cline{3-10}
& & MetaGPT \cite{hong2023metagpt}& \color{orange}{\xmark} & \green{\cmark} & \green{\cmark} & \green{\cmark} & \green{\cmark} & \green{\cmark} & Programming (T) \\ \cline{3-10}
& & Mobile-Agent-V2 \cite{wang2024mobileV2} & \green{\cmark} & \green{\cmark} & \color{orange}{\xmark} & \green{\cmark} & \green{\cmark} & \green{\cmark} & Device Control (T) \\ 
\cline{2-10}
% \midrule

% ================= Single Agent, End-to-End ==================

& \multirow{5}{*}{\begin{tabular}{c}End-to-End\\Paradigm\end{tabular}} 
& RT-2 \cite{brohan2023rt} & \multicolumn{6}{c|}{\multirow{3}{*}{Vision-Language-Action Model}} & Robot Control (E) \\ \cline{3-3} \cline{10-10}
& & OpenVLA \cite{kim2024openvla} & \multicolumn{6}{c|}{} & Robot Control (E) \\ \cline{3-3} \cline{10-10}
& & $\pi_0$ \cite{black2024pi_0} & \multicolumn{6}{c|}{} & Robot Control (E) \\ \cline{3-10}
& & \multirow{2}{*}{\begin{tabular}{c}Octo \cite{team2024octo}\\PaLM-E \cite{driess2023palme}\end{tabular}} & \multicolumn{6}{c|}{\multirow{2}{*}{Vision-Language Model + Exec Policy}} & Robot Control (E) \\ \cline{3-3} \cline{10-10}
& &  & \multicolumn{6}{c|}{} & Robot Control (E) \\ 
\hline



% ================ Multi-agent, Centralized =====================
\multirow{17}{*}{\begin{tabular}{c}Multi-\\Agent\end{tabular}} 
& \multirow{8}{*}{\begin{tabular}{c}Centralized\\Paradigm\end{tabular}} 
& LLaMAC \cite{zhang2023controlling} & \color{orange}{\xmark} & \green{\cmark} & \green{\cmark} & \green{\cmark} & \color{orange}{\xmark} & \green{\cmark} & Simulation (V) \\ \cline{3-10}
& & MindAgent \cite{gong2023mindagent} & \color{orange}{\xmark} & \green{\cmark} & \green{\cmark} & \green{\cmark}  & \color{orange}{\xmark} & \green{\cmark} & Simulation (V) \\ \cline{3-10}
& & OLA \cite{guo2024embodied} & \color{orange}{\xmark} & \green{\cmark} & \green{\cmark} & \green{\cmark} & \green{\cmark} & \green{\cmark} & Simulation (V) \\ \cline{3-10}
& & ALGPT \cite{zhou2024algpt} & \green{\cmark} & \green{\cmark} & \green{\cmark} & \green{\cmark} & \color{orange}{\xmark} & \green{\cmark} & Navigation (V) \\ \cline{3-10}
& & CMAS \cite{chen2024scalable} & \green{\cmark} & \green{\cmark} & \green{\cmark} & \green{\cmark}  & \color{orange}{\xmark} & \green{\cmark} & Simulation (V) \\ \cline{3-10}
& & ReAd \cite{zhang2024towards} & \color{orange}{\xmark} & \green{\cmark} & \green{\cmark} & \color{orange}{\xmark} & \green{\cmark} & \green{\cmark} & Simulation (V) \\ \cline{3-10}
& & Co-NavGPT \cite{yu2023co}& \green{\cmark} & \green{\cmark} & \green{\cmark} & \color{orange}{\xmark} & \color{orange}{\xmark} & \green{\cmark}  & Navigation (V) \\ \cline{3-10}
& & COHERENT \cite{liu2024coherent} & \green{\cmark} & \green{\cmark} & \green{\cmark} & \green{\cmark} & \green{\cmark} & \green{\cmark} & Simulation (V) \\ \cline{2-10}

% ================ Multi-agent, Decentralized =====================
& \multirow{9}{*}{\begin{tabular}{c}Decentralized\\Paradigm\end{tabular}} 
& DMAS \cite{chen2024scalable} & \green{\cmark} & \green{\cmark} & \green{\cmark} & \green{\cmark} & \color{orange}{\xmark} & \green{\cmark} & Simulation (V) \\ \cline{3-10}
& & HMAS \cite{chen2024scalable} & \green{\cmark} & \green{\cmark} & \green{\cmark} & \green{\cmark} & \green{\cmark} & \green{\cmark} & Simulation (V) \\ \cline{3-10}
& & AGA \cite{yu2024affordable} & \green{\cmark} & \green{\cmark} & \green{\cmark} & \green{\cmark} & \green{\cmark} & \green{\cmark} & Simulation (V) \\ \cline{3-10}
& & CoELA \cite{zhang2024building}& \green{\cmark} & \green{\cmark} & \green{\cmark} & \green{\cmark} & \color{orange}{\xmark} & \green{\cmark} & Simulation (V) \\ \cline{3-10}
& & FMA \cite{lu2023building} & \color{orange}{\xmark} & \green{\cmark} & \green{\cmark} & \green{\cmark} & \green{\cmark} & \green{\cmark} & Programming (T) \\ \cline{3-10}
& & COMBO \cite{zhang2024building}& \green{\cmark} & \green{\cmark} & \green{\cmark} & \green{\cmark} & \color{orange}{\xmark} & \green{\cmark} & Simulation (V) \\ \cline{3-10}
& & RoCo \cite{mandi2024roco}& \green{\cmark} & \green{\cmark} & \green{\cmark} & \green{\cmark} & \green{\cmark} & \green{\cmark} & Simulation (V) \\ \cline{3-10}
& & AgentVerse \cite{chen2023agentverse} & \color{orange}{\xmark} & \green{\cmark} & \green{\cmark} & \color{orange}{\xmark} & \color{orange}{\xmark} & \green{\cmark} & Simulation (V) \\ \cline{3-10}
& & KoMA \cite{jiang2024koma} & \color{orange}{\xmark} & \green{\cmark} & \green{\cmark} & \green{\cmark} & \green{\cmark} & \green{\cmark} & Simulation (V) \\
\hline   
% \bottomrule
\end{tabular}
}
\vspace{-10pt}
\end{table}
 
